DIALKI: Knowledge Identification in Conversational Systems through Dialogue-Document Contextualization

Identifying relevant knowledge to be used in conversational systems that are grounded in long documents is critical to effective response generation. We introduce a knowledge identification model that leverages the document structure to provide dialogue-contextualized passage encodings and better locate knowledge relevant to the conversation. An auxiliary loss captures the history of dialogue-document connections. We demonstrate the effectiveness of our model on two document-grounded conversational datasets and provide analyses showing generalization to unseen documents and long dialogue contexts.

==> tables/doc2dial_ablation.tex <==
\begin{table*}[!htp]\centering
\begin{tabular}{lccccccc}\toprule
\multirow{2}{*}{\textbf{Method}} &\multicolumn{2}{c}{\textbf{Overall}} &\multicolumn{2}{c}{\textbf{Seen}} &\multicolumn{2}{c}{\textbf{Unseen}} \\
&EM &F1 &EM &F1 &EM &F1 \\\midrule
single-doc (token-level) &42.20 &58.13 &48.33 &61.13 &36.96 &55.56 \\
single-doc &46.27 &59.26 &54.35 &63.51 &39.38 &55.64 \\
multi-sentence &59.49 &68.76 &63.64 &71.58 &55.95 &66.35 \\
multi-passage &60.42 &71.19 &64.24 &72.31 &57.16 &70.23 \\
\; $+ \mathcal{L}_{\text{hist}}$ &62.97 &72.85 &66.54 &73.93 &59.92 &71.93 \\
\; $+ \mathcal{L}_{\text{hist}} +$ span ctx &63.8 &73.43 &\textbf{67.69} &74.78 &60.48 &72.27 \\
\; $+ \mathcal{L}_{\text{adv}}$ &64.38 &73.78 &66.21 &73.94 &62.81 &73.65 \\
\; $+ \mathcal{L}_{\text{hist}} + \mathcal{L}_{\text{adv}} +$ span ctx &\textbf{65.86} &\textbf{74.78} &67.58 &\textbf{74.91} &\textbf{64.4} &\textbf{74.67} \\
\bottomrule
\end{tabular}
\caption{The ablation results of Doc2Dial dev set.}
\label{tab:doc2dial_ablation}
\end{table*}

==> tables/history_loss_effect.tex <==
\begin{table}%[!htp]
\centering
\small
\begin{tabular}{lcccc}\toprule
\multirow{2}{*}{\textbf{History Labels}} &\multicolumn{2}{c}{\textbf{Doc2Dial}} \\
&EM &F1 \\\midrule
all turns &63.0 &72.9 \\
all agent turns &62.7 &72.8  \\
50\% agent turns &62.4 &72.6 \\
no turns &60.4 &71.2 \\
\bottomrule
\end{tabular}
\caption{Results of \ours ($\mathcal{L}_{next}$,$\mathcal{L}_{hist}$) on Doc2Dial dev set with different history knowledge labels.}
\label{tab:hist_loss_effect}
\end{table}

==> tables/wow_ablation.tex <==
\begin{table*}[!htp]\centering
\begin{tabular}{lcccccccc}\toprule
\multirow{2}{*}{\textbf{Method}} &\multicolumn{2}{c}{\textbf{Overall}} &\multicolumn{2}{c}{\textbf{Seen}}  &\multicolumn{2}{c}{\textbf{Unseen}}\\
&EM &F1 &EM &F1 &EM &F1 \\\midrule
multi-sentence &29.21 &36.96 &32.37 &39.7 &26.1 &34.26 \\
multi-passage &31.50 &39.70 &33.26 &41.11 &29.77 &38.31 \\
\; $+ \mathcal{L}_{\text{hist}}$ &33.64 &41.58 &35.09 &42.71 &32.21 &40.46 \\
\; $+ \mathcal{L}_{\text{hist}} +$ span ctx &33.62 &41.53 &35.16 &42.77 &32.11 &40.3 \\
\; $+ \mathcal{L}_{\text{adv}}$ &32.87 &40.83 &34.63 &42.19 &31.14 &39.49 \\
\; $+ \mathcal{L}_{\text{hist}} + \mathcal{L}_{\text{adv}} +$ span ctx & \textbf{34.23} & \textbf{42.06} &\textbf{35.92} &\textbf{43.46} &\textbf{32.57} &\textbf{40.68} \\
\bottomrule
\end{tabular}
\caption{The ablation results of wizard of wikipedia test set.}
\label{tab:wow_ablation}
\end{table*}
